Disequilibrium Chemistry, Diabatic Thermal Structure, and Clouds in the Atmosphere of COCONUTS-2b

Located 10.888 pc from Earth, COCONUTS-2b is a planetary-mass companion to a young (150-800 Myr) M3 star, with a wide orbital separation (6471 au) and a low companion-to-host mass ratio ($0.021\pm0.005$). We have studied the atmospheric properties of COCONUTS-2b using newly acquired 1.0-2.5 $\mu$m spectroscopy from Gemini/Flamingos-2. The spectral type of COCONUTS-2b is refined to T$9.5 \pm 0.5$ based on comparisons with T/Y dwarf spectral templates. We have conducted an extensive forward-modeling analysis, comparing the near-infrared spectrum and mid-infrared broadband photometry with sixteen state-of-the-art atmospheric model grids developed for brown dwarfs and self-luminous exoplanets near the T/Y transition. The PH$_{3}$-free ATMO2020++, ATMO2020++, and Exo-REM models best match the specific observations of COCONUTS-2b, regardless of variations in the input spectrophotometry. This analysis suggests the presence of disequilibrium chemistry, along with a diabatic thermal structure and/or clouds, in the atmosphere of COCONUTS-2b. All models predict fainter $Y$-band fluxes than observed, highlighting uncertainties in the alkali chemistry models and opacities. We determine a bolometric luminosity of $\log{(L_{\rm bol}/L_{\odot})}=-6.18$ dex, with a 0.5 dex-wide range of $[-6.43,-5.93]$ dex that accounts for various assumptions of models. Using thermal evolution models, we derive an effective temperature of $T_{\rm eff}=483^{+44}_{-53}$ K, a surface gravity of $\log{(g)}=4.19^{+0.18}_{-0.13}$ dex, a radius of $R=1.11^{+0.03}_{-0.04}$ R$_{\rm Jup}$, and a mass of $M=8 \pm 2$ M$_{\rm Jup}$. Various atmospheric model grids consistently indicate that COCONUTS-2b's atmosphere has sub- or near-solar metallicity and C/O. These findings provide valuable insights into COCONUTS-2b's formation history and the potential outward migration to its current wide orbit.

==> C2b_fm_params_key_runs.tex <==
\renewcommand{\arraystretch}{1.25} 
{ 
\begin{deluxetable*}{lcccccccccc}
\setlength{\tabcolsep}{1.3pt} 
\tablecaption{Atmospheric properties of COCONUTS-2b (Gemini/F2 spectrum and $W1$/$W2$/[3.6]/[4.5] photometry)} \label{tab:fm_params_key_runs} 
\tablehead{ \multicolumn{1}{l}{Atmospheric Model Grid}   &   \multicolumn{1}{c}{$\Delta$BIC}\tablenotemark{\scriptsize a}   &   \multicolumn{1}{c}{$T_{\rm eff}$}   &   \multicolumn{1}{c}{$\log{(g)}$}   &   \multicolumn{1}{c}{[M/H]\tablenotemark{\scriptsize b}}   &   \multicolumn{1}{c}{C/O\tablenotemark{\scriptsize b}}   &   \multicolumn{1}{c}{$f_{\rm sed}$\tablenotemark{\scriptsize b}}   &   \multicolumn{1}{c}{$\log{(K_{\rm zz})}$\tablenotemark{\scriptsize b}}   &   \multicolumn{1}{c}{$R$}   &   \multicolumn{1}{c}{$\log{(b)}$}   &   \multicolumn{1}{c}{$\log{(L_{\rm bol}/L_{\odot})}$\tablenotemark{\scriptsize c}}    \\ 
\multicolumn{1}{l}{}   &   \multicolumn{1}{c}{}   &   \multicolumn{1}{c}{(K)}   &   \multicolumn{1}{c}{(dex)}   &   \multicolumn{1}{c}{(dex)}   &   \multicolumn{1}{c}{}   &   \multicolumn{1}{c}{}   &   \multicolumn{1}{c}{(cm$^{2}/$s)}   &   \multicolumn{1}{c}{(R$_{\rm Jup}$)}   &   \multicolumn{1}{c}{(erg s$^{-1}$ cm$^{-2}$ \AA$^{-1}$)}   &   \multicolumn{1}{c}{(dex)}  } 
\startdata 
\multicolumn{11}{c}{disequilibrium chemistry + diabatic thermal structure + no clouds}   \\ 
\hline   
\texttt{PH$_{3}$-free ATMO2020++} & $0$ & $545.5^{+3.3}_{-3.2}$ & $4.174^{+0.024}_{-0.015}$ & $-0.152^{+0.012}_{-0.010}$ & ($0.55$) & $\dots$ & ($6.65^{+0.03}_{-0.05}$) & $0.878^{+0.014}_{-0.015}$ & $-18.52^{+0.06}_{-0.07}$ & $-6.179^{+0.005}_{-0.005}$  \\ 
\texttt{ATMO2020++} & $6$ & $534.5^{+3.9}_{-3.8}$ & $4.220^{+0.036}_{-0.039}$ & $-0.209^{+0.025}_{-0.021}$ & ($0.55$) & $\dots$ & ($6.56^{+0.08}_{-0.07}$) & $0.933^{+0.020}_{-0.020}$ & $-18.54^{+0.06}_{-0.08}$ & $-6.161^{+0.006}_{-0.006}$  \\ 
\hline   
\multicolumn{11}{c}{disequilibrium chemistry + clouds}   \\ 
\hline   
\texttt{Exo-REM} & $111$ & $449.9^{+0.4}_{-0.7}$ & $3.348^{+0.004}_{-0.006}$ & $-0.001^{+0.008}_{-0.009}$ & $0.400^{+0.001}_{-0.000}$ & (microphys.) & (profile) & $1.902^{+0.012}_{-0.011}$ & $-18.34^{+0.04}_{-0.04}$ & $-5.849^{+0.004}_{-0.004}$  \\ 
\hline   
\multicolumn{11}{c}{disequilibrium chemistry + no clouds}   \\ 
\hline   
\texttt{LB23 Clear NEQ} & $557$ & $463.2^{+1.0}_{-1.0}$ & $3.758^{+0.012}_{-0.006}$ & $-0.309^{+0.021}_{-0.021}$ & (0.537) & $\dots$ & (profile) & $1.149^{+0.009}_{-0.009}$ & $-18.28^{+0.04}_{-0.04}$ & $-6.225^{+0.004}_{-0.004}$  \\ 
\texttt{Sonora Elf Owl} & $638$ & $472.7^{+4.6}_{-3.4}$ & $3.235^{+0.007}_{-0.003}$ & $-0.265^{+0.034}_{-0.040}$ & $0.505^{+0.007}_{-0.004}$ & $\dots$ & $8.96^{+0.03}_{-0.06}$ & $1.106^{+0.025}_{-0.031}$ & $-18.33^{+0.04}_{-0.05}$ & $-6.224^{+0.007}_{-0.008}$  \\ 
\texttt{ATMO2020 NEQ strong} & $832$ & $445.6^{+2.6}_{-2.6}$ & $4.810^{+0.035}_{-0.036}$ & (0) & ($0.55$) & $\dots$ & ($5.38^{+0.07}_{-0.07}$) & $1.145^{+0.022}_{-0.022}$ & $-18.38^{+0.04}_{-0.05}$ & $-6.293^{+0.007}_{-0.007}$  \\ 
\texttt{ATMO2020 NEQ weak} & $886$ & $461.7^{+2.4}_{-2.5}$ & $4.808^{+0.038}_{-0.038}$ & (0) & ($0.55$) & $\dots$ & ($3.38^{+0.08}_{-0.08}$) & $1.023^{+0.016}_{-0.016}$ & $-18.40^{+0.05}_{-0.05}$ & $-6.327^{+0.005}_{-0.005}$  \\ 
\hline   
\multicolumn{11}{c}{equilibrium chemistry + clouds}   \\ 
\hline   
\texttt{Linder19 Cloudy} & $402$ & $655.2^{+4.6}_{-5.6}$ & $3.294^{+0.088}_{-0.083}$ & $-0.398^{+0.004}_{-0.002}$ & ($0.55$) & $0.93^{+0.12}_{-0.07}$ & $\dots$ & $0.586^{+0.006}_{-0.006}$ & $-18.11^{+0.03}_{-0.04}$ & $-6.226^{+0.011}_{-0.015}$  \\ 
\texttt{Morley12} & $993$ & $570.3^{+4.9}_{-4.8}$ & $4.720^{+0.054}_{-0.053}$ & (0) & ($0.497$) & $4.97^{+0.02}_{-0.03}$ & $\dots$ & $0.621^{+0.010}_{-0.010}$ & $-18.02^{+0.02}_{-0.02}$ & $-6.406^{+0.005}_{-0.005}$  \\ 
\texttt{Morley14}\tablenotemark{\scriptsize d} & $1522$ & $449.9^{+0.1}_{-0.1}$ & $4.205^{+0.036}_{-0.035}$ & (0) & ($0.497$) & (5) & $\dots$ & $1.024^{+0.005}_{-0.004}$ & $-17.99^{+0.02}_{-0.02}$ & $-6.360^{+0.004}_{-0.004}$  \\ 
\hline   
\multicolumn{11}{c}{equilibrium chemistry + no clouds}   \\ 
\hline   
\texttt{LB23 Clear CEQ} (M1)\tablenotemark{\scriptsize e} & $881$ & $561.7^{+0.7}_{-0.9}$ & $4.630^{+0.013}_{-0.015}$ & $-0.261^{+0.012}_{-0.013}$ & (0.537) & $\dots$ & $\dots$ & $0.630^{+0.004}_{-0.004}$ & $-18.10^{+0.02}_{-0.02}$ & $-6.408^{+0.004}_{-0.004}$  \\ 
\texttt{LB23 Clear CEQ} (M2)\tablenotemark{\scriptsize e} & $886$ & $559.7^{+0.7}_{-0.7}$ & $4.415^{+0.018}_{-0.012}$ & $-0.311^{+0.012}_{-0.012}$ & (0.537) & $\dots$ & $\dots$ & $0.633^{+0.004}_{-0.004}$ & $-18.12^{+0.02}_{-0.02}$ & $-6.411^{+0.004}_{-0.004}$  \\ 
\texttt{Linder19 Clear} & $915$ & $487.6^{+1.6}_{-1.6}$ & $3.223^{+0.051}_{-0.051}$ & $-0.394^{+0.010}_{-0.005}$ & ($0.55$) & $\dots$ & $\dots$ & $0.863^{+0.008}_{-0.008}$ & $-18.37^{+0.04}_{-0.05}$ & $-6.379^{+0.004}_{-0.004}$  \\ 
\texttt{ATMO2020 CEQ} & $972$ & $493.0^{+2.0}_{-1.9}$ & $5.178^{+0.042}_{-0.041}$ & (0) & ($0.55$) & $\dots$ & $\dots$ & $0.834^{+0.008}_{-0.008}$ & $-18.18^{+0.03}_{-0.03}$ & $-6.387^{+0.004}_{-0.004}$  \\ 
\texttt{Sonora Bobcat} & $1189$ & $530.4^{+2.7}_{-2.7}$ & $5.494^{+0.005}_{-0.010}$ & $0.102^{+0.020}_{-0.021}$ & ($0.458$) & $\dots$ & $\dots$ & $0.700^{+0.008}_{-0.008}$ & $-18.19^{+0.03}_{-0.03}$ & $-6.414^{+0.004}_{-0.004}$  \\ 
\enddata 
\tablenotetext{a}{This column lists the BIC value of each model grid relative to that of the \texttt{PH$_{3}$-free ATMO2020++} models.}  
\tablenotetext{b}{Values inside parentheses are fixed by the model grids. In particular, the $\log{(K_{\rm zz})}$ values of the \texttt{ATMO2020}, \texttt{ATMO2020++}, and \texttt{PH$_{3}$-free ATMO2020++} modeling results are linearly interpolated from the inferred $\log{(g)}$ based on Figure~1 of Phillips et al. (2021). }  
\tablenotetext{c}{The bolometric luminosity is computed based on Equation~\ref{eq:lbol} that accounts for the offsets between observed fluxes and the fitted models}  
\tablenotetext{d}{The inferred $T_{\rm eff}$ based on \texttt{Morley14} models is pinned at the maximum grid value at 450~K.}  
\tablenotetext{e}{The parameter posteriors inferred by the \texttt{LB23 Clear CEQ} grid exhibit two modes, with the corresponding results labeled as ``M1'' and ``M2''.   }  
\end{deluxetable*} 
} 


==> C2b_noY_fm_params_key_runs.tex <==
\renewcommand{\arraystretch}{1.18} 
{ 
\begin{deluxetable*}{lcccccccccc}
\setlength{\tabcolsep}{1.3pt} 
\tablecaption{Atmospheric properties of COCONUTS-2b ($Y$-band spectrum excluded)} \label{tab:fm_params_key_runs_noY} 
\tablehead{ \multicolumn{1}{l}{Atmospheric Model Grid}   &   \multicolumn{1}{c}{$\Delta$BIC}\tablenotemark{\scriptsize a}   &   \multicolumn{1}{c}{$T_{\rm eff}$}   &   \multicolumn{1}{c}{$\log{(g)}$}   &   \multicolumn{1}{c}{[M/H]\tablenotemark{\scriptsize b}}   &   \multicolumn{1}{c}{C/O\tablenotemark{\scriptsize c}}   &   \multicolumn{1}{c}{$f_{\rm sed}$\tablenotemark{\scriptsize b}}   &   \multicolumn{1}{c}{$\log{(K_{\rm zz})}$\tablenotemark{\scriptsize b}}   &   \multicolumn{1}{c}{$R$}   &   \multicolumn{1}{c}{$\log{(b)}$}   &   \multicolumn{1}{c}{$\log{(L_{\rm bol}/L_{\odot})}$\tablenotemark{\scriptsize c}}    \\ 
\multicolumn{1}{l}{}   &   \multicolumn{1}{c}{}   &   \multicolumn{1}{c}{(K)}   &   \multicolumn{1}{c}{(dex)}   &   \multicolumn{1}{c}{(dex)}   &   \multicolumn{1}{c}{}   &   \multicolumn{1}{c}{}   &   \multicolumn{1}{c}{(cm$^{2}/$s)}   &   \multicolumn{1}{c}{(R$_{\rm Jup}$)}   &   \multicolumn{1}{c}{(erg s$^{-1}$ cm$^{-2}$ \AA$^{-1}$)}   &   \multicolumn{1}{c}{(dex)}  } 
\startdata 
\multicolumn{11}{c}{disequilibrium chemistry + diabatic thermal structure + no clouds}   \\ 
\hline   
\texttt{ATMO2020++} (M1)\tablenotemark{\scriptsize d} & $-34$ & $563.1^{+2.8}_{-2.9}$ & $4.611^{+0.015}_{-0.014}$ & $-0.105^{+0.012}_{-0.012}$ & ($0.55$) & $\dots$ & ($5.78^{+0.03}_{-0.03}$) & $0.795^{+0.011}_{-0.011}$ & $-18.60^{+0.07}_{-0.09}$ & $-6.215^{+0.005}_{-0.005}$  \\ 
\texttt{ATMO2020++} (M2)\tablenotemark{\scriptsize d} & $-33$ & $555.0^{+2.4}_{-2.5}$ & $4.682^{+0.018}_{-0.014}$ & $0.024^{+0.013}_{-0.012}$ & ($0.55$) & $\dots$ & ($5.64^{+0.03}_{-0.04}$) & $0.826^{+0.011}_{-0.011}$ & $-18.68^{+0.09}_{-0.14}$ & $-6.207^{+0.005}_{-0.005}$  \\ 
\texttt{PH$_{3}$-free ATMO2020++} & $0$ & $549.3^{+2.8}_{-3.1}$ & $4.223^{+0.027}_{-0.028}$ & $-0.155^{+0.016}_{-0.015}$ & ($0.55$) & $\dots$ & ($6.55^{+0.06}_{-0.05}$) & $0.855^{+0.014}_{-0.013}$ & $-18.55^{+0.06}_{-0.08}$ & $-6.194^{+0.005}_{-0.006}$  \\ 
\hline   
\multicolumn{11}{c}{disequilibrium chemistry + clouds}   \\ 
\hline   
\texttt{Exo-REM} (M1)\tablenotemark{\scriptsize d} & $209$ & $452.9^{+1.8}_{-1.9}$ & $3.332^{+0.011}_{-0.010}$ & $-0.132^{+0.010}_{-0.009}$ & $0.435^{+0.002}_{-0.003}$ & (microphys.) & (profile) & $1.887^{+0.025}_{-0.024}$ & $-18.38^{+0.04}_{-0.05}$ & $-5.845^{+0.005}_{-0.006}$  \\ 
\texttt{Exo-REM} (M2)\tablenotemark{\scriptsize d} & $214$ & $450.0^{+0.7}_{-0.9}$ & $3.340^{+0.005}_{-0.008}$ & $-0.011^{+0.010}_{-0.018}$ & $0.400^{+0.001}_{-0.000}$ & (microphys.) & (profile) & $1.904^{+0.014}_{-0.012}$ & $-18.41^{+0.04}_{-0.05}$ & $-5.848^{+0.005}_{-0.005}$  \\ 
\hline   
\multicolumn{11}{c}{disequilibrium chemistry + no clouds}   \\ 
\hline   
\texttt{Sonora Elf Owl} & $605$ & $469.2^{+2.7}_{-2.7}$ & $3.243^{+0.021}_{-0.009}$ & $-0.276^{+0.027}_{-0.028}$ & $0.503^{+0.005}_{-0.003}$ & $\dots$ & $8.98^{+0.01}_{-0.03}$ & $1.116^{+0.021}_{-0.020}$ & $-18.40^{+0.05}_{-0.05}$ & $-6.233^{+0.006}_{-0.007}$  \\ 
\texttt{LB23 Clear NEQ} & $638$ & $464.7^{+1.1}_{-1.2}$ & $3.791^{+0.013}_{-0.020}$ & $-0.320^{+0.021}_{-0.022}$ & (0.537) & $\dots$ & (profile) & $1.131^{+0.010}_{-0.010}$ & $-18.31^{+0.04}_{-0.04}$ & $-6.237^{+0.004}_{-0.004}$  \\ 
\texttt{ATMO2020 NEQ strong} (M1)\tablenotemark{\scriptsize d} & $903$ & $465.7^{+2.7}_{-2.7}$ & $5.130^{+0.033}_{-0.033}$ & (0) & ($0.55$) & $\dots$ & ($4.74^{+0.07}_{-0.07}$) & $1.000^{+0.014}_{-0.014}$ & $-18.32^{+0.04}_{-0.04}$ & $-6.337^{+0.004}_{-0.004}$  \\ 
\texttt{ATMO2020 NEQ strong} (M2)\tablenotemark{\scriptsize d} & $908$ & $449.1^{+2.3}_{-2.3}$ & $4.896^{+0.031}_{-0.032}$ & (0) & ($0.55$) & $\dots$ & ($5.21^{+0.06}_{-0.06}$) & $1.101^{+0.020}_{-0.017}$ & $-18.40^{+0.04}_{-0.05}$ & $-6.317^{+0.007}_{-0.006}$  \\ 
\texttt{ATMO2020 NEQ weak} (M1)\tablenotemark{\scriptsize d} & $942$ & $476.4^{+2.1}_{-2.2}$ & $5.139^{+0.033}_{-0.035}$ & (0) & ($0.55$) & $\dots$ & ($2.72^{+0.07}_{-0.07}$) & $0.933^{+0.011}_{-0.011}$ & $-18.32^{+0.04}_{-0.04}$ & $-6.357^{+0.004}_{-0.004}$  \\ 
\texttt{ATMO2020 NEQ weak} (M2)\tablenotemark{\scriptsize d} & $951$ & $463.8^{+2.4}_{-2.4}$ & $4.900^{+0.039}_{-0.039}$ & (0) & ($0.55$) & $\dots$ & ($3.20^{+0.08}_{-0.08}$) & $0.999^{+0.015}_{-0.016}$ & $-18.41^{+0.05}_{-0.05}$ & $-6.345^{+0.004}_{-0.005}$  \\ 
\hline   
\multicolumn{11}{c}{equilibrium chemistry + clouds}   \\ 
\hline   
\texttt{Linder19 Cloudy} & $504$ & $640.4^{+3.2}_{-3.7}$ & $3.597^{+0.040}_{-0.042}$ & $-0.395^{+0.007}_{-0.003}$ & ($0.55$) & $0.90^{+0.06}_{-0.04}$ & $\dots$ & $0.593^{+0.005}_{-0.005}$ & $-18.17^{+0.03}_{-0.03}$ & $-6.253^{+0.009}_{-0.011}$  \\ 
\texttt{Morley12} & $1044$ & $580.9^{+4.7}_{-4.6}$ & $4.944^{+0.050}_{-0.054}$ & (0) & ($0.497$) & $4.93^{+0.05}_{-0.10}$ & $\dots$ & $0.599^{+0.009}_{-0.009}$ & $-18.01^{+0.02}_{-0.02}$ & $-6.410^{+0.005}_{-0.004}$  \\ 
\texttt{Morley14}\tablenotemark{\scriptsize e} & $1687$ & $449.9^{+0.1}_{-0.1}$ & $4.394^{+0.048}_{-0.041}$ & (0) & ($0.497$) & (5) & $\dots$ & $1.012^{+0.005}_{-0.004}$ & $-17.99^{+0.02}_{-0.02}$ & $-6.372^{+0.004}_{-0.004}$  \\ 
\hline   
\multicolumn{11}{c}{equilibrium chemistry + no clouds}   \\ 
\hline   
\texttt{LB23 Clear CEQ} (M1)\tablenotemark{\scriptsize d} & $987$ & $550.1^{+1.3}_{-1.1}$ & $4.995^{+0.004}_{-0.009}$ & $-0.167^{+0.014}_{-0.015}$ & (0.537) & $\dots$ & $\dots$ & $0.650^{+0.004}_{-0.004}$ & $-18.08^{+0.02}_{-0.02}$ & $-6.420^{+0.004}_{-0.004}$  \\ 
\texttt{LB23 Clear CEQ} (M2)\tablenotemark{\scriptsize d} & $990$ & $559.1^{+1.4}_{-2.6}$ & $4.667^{+0.028}_{-0.019}$ & $-0.279^{+0.020}_{-0.016}$ & (0.537) & $\dots$ & $\dots$ & $0.634^{+0.006}_{-0.004}$ & $-18.10^{+0.02}_{-0.02}$ & $-6.415^{+0.004}_{-0.005}$  \\ 
\texttt{ATMO2020 CEQ} & $1047$ & $495.6^{+2.0}_{-2.0}$ & $5.351^{+0.046}_{-0.045}$ & (0) & ($0.55$) & $\dots$ & $\dots$ & $0.822^{+0.009}_{-0.009}$ & $-18.15^{+0.03}_{-0.03}$ & $-6.396^{+0.004}_{-0.004}$  \\ 
\texttt{Linder19 Clear} & $1051$ & $483.0^{+3.1}_{-2.8}$ & $3.539^{+0.064}_{-0.081}$ & $-0.389^{+0.019}_{-0.008}$ & ($0.55$) & $\dots$ & $\dots$ & $0.876^{+0.013}_{-0.014}$ & $-18.35^{+0.04}_{-0.05}$ & $-6.386^{+0.004}_{-0.004}$  \\ 
\texttt{Sonora Bobcat} & $1340$ & $547.3^{+3.6}_{-3.5}$ & $5.322^{+0.061}_{-0.062}$ & $-0.123^{+0.027}_{-0.027}$ & ($0.458$) & $\dots$ & $\dots$ & $0.665^{+0.008}_{-0.008}$ & $-18.11^{+0.03}_{-0.03}$ & $-6.410^{+0.005}_{-0.005}$  \\ 
\enddata 
\tablenotetext{a}{This column lists the BIC value of each model grid relative to that of the \texttt{PH$_{3}$-free ATMO2020++} models.}  
\tablenotetext{b}{Values inside parentheses are fixed by the model grids. In particular, the $\log{(K_{\rm zz})}$ values of the \texttt{ATMO2020}, \texttt{ATMO2020++}, and \texttt{PH$_{3}$-free ATMO2020++} modeling results are linearly interpolated from the inferred $\log{(g)}$ based on Figure~1 of Phillips et al. (2021). }  
\tablenotetext{c}{The bolometric luminosity is computed based on Equation~\ref{eq:lbol} that accounts for the offsets between observed fluxes and the fitted models}  
\tablenotetext{d}{The parameter posteriors inferred by these model grids exhibit two modes, with the corresponding results labeled as ``M1'' and ``M2''.  }  
\tablenotetext{e}{The inferred $T_{\rm eff}$ based on \texttt{Morley14} models is pinned at the maximum grid value at 450~K.}  
\end{deluxetable*} 
} 


==> C2b_w3_fm_params_key_runs.tex <==
\renewcommand{\arraystretch}{1.25} 
{ 
\begin{deluxetable*}{lcccccccccc}
\setlength{\tabcolsep}{1.3pt} 
\tablecaption{Atmospheric properties of COCONUTS-2b ($W3$ photometry included)} \label{tab:fm_params_key_runs_w3} 
\tablehead{ \multicolumn{1}{l}{Atmospheric Model Grid\tablenotemark{\scriptsize a}}   &   \multicolumn{1}{c}{$\Delta$BIC}\tablenotemark{\scriptsize b}   &   \multicolumn{1}{c}{$T_{\rm eff}$}   &   \multicolumn{1}{c}{$\log{(g)}$}   &   \multicolumn{1}{c}{[M/H]\tablenotemark{\scriptsize c}}   &   \multicolumn{1}{c}{C/O\tablenotemark{\scriptsize c}}   &   \multicolumn{1}{c}{$f_{\rm sed}$\tablenotemark{\scriptsize c}}   &   \multicolumn{1}{c}{$\log{(K_{\rm zz})}$\tablenotemark{\scriptsize c}}   &   \multicolumn{1}{c}{$R$}   &   \multicolumn{1}{c}{$\log{(b)}$}   &   \multicolumn{1}{c}{$\log{(L_{\rm bol}/L_{\odot})}$\tablenotemark{\scriptsize d}}    \\ 
\multicolumn{1}{l}{}   &   \multicolumn{1}{c}{}   &   \multicolumn{1}{c}{(K)}   &   \multicolumn{1}{c}{(dex)}   &   \multicolumn{1}{c}{(dex)}   &   \multicolumn{1}{c}{}   &   \multicolumn{1}{c}{}   &   \multicolumn{1}{c}{(cm$^{2}/$s)}   &   \multicolumn{1}{c}{(R$_{\rm Jup}$)}   &   \multicolumn{1}{c}{(erg s$^{-1}$ cm$^{-2}$ \AA$^{-1}$)}   &   \multicolumn{1}{c}{(dex)}  } 
\startdata 
\multicolumn{10}{c}{disequilibrium chemistry + diabatic thermal structure + no clouds}   \\ 
\hline   
\texttt{PH$_{3}$-free ATMO2020++} & $0$ & $544.6^{+3.3}_{-3.2}$ & $4.170^{+0.022}_{-0.014}$ & $-0.151^{+0.012}_{-0.010}$ & ($0.55$) & $\dots$ & ($6.66^{+0.03}_{-0.04}$) & $0.883^{+0.014}_{-0.015}$ & $-18.52^{+0.06}_{-0.07}$ & $-6.177^{+0.005}_{-0.005}$  \\ 
\texttt{ATMO2020++} & $4$ & $533.2^{+3.9}_{-3.9}$ & $4.212^{+0.034}_{-0.041}$ & $-0.208^{+0.024}_{-0.021}$ & ($0.55$) & $\dots$ & ($6.58^{+0.08}_{-0.07}$) & $0.940^{+0.020}_{-0.020}$ & $-18.54^{+0.06}_{-0.08}$ & $-6.159^{+0.007}_{-0.006}$  \\ 
\hline   
\multicolumn{10}{c}{disequilibrium chemistry + clouds}   \\ 
\hline   
\texttt{Exo-REM} & $105$ & $449.9^{+0.4}_{-0.6}$ & $3.349^{+0.004}_{-0.006}$ & $-0.001^{+0.008}_{-0.009}$ & $0.400^{+0.000}_{-0.000}$ & (microphys.) & (profile) & $1.899^{+0.012}_{-0.011}$ & $-18.34^{+0.04}_{-0.05}$ & $-5.850^{+0.004}_{-0.004}$  \\ 
\hline   
\multicolumn{10}{c}{disequilibrium chemistry + no clouds}   \\ 
\hline   
\texttt{LB23 Clear NEQ} & $562$ & $463.1^{+1.0}_{-1.0}$ & $3.759^{+0.012}_{-0.006}$ & $-0.304^{+0.021}_{-0.021}$ & (0.537) & $\dots$ & (profile) & $1.151^{+0.009}_{-0.009}$ & $-18.28^{+0.04}_{-0.04}$ & $-6.225^{+0.004}_{-0.004}$  \\ 
\texttt{ATMO2020 NEQ strong} & $842$ & $444.9^{+2.6}_{-2.6}$ & $4.799^{+0.036}_{-0.036}$ & (0) & ($0.55$) & $\dots$ & ($5.40^{+0.07}_{-0.07}$) & $1.152^{+0.022}_{-0.022}$ & $-18.38^{+0.04}_{-0.05}$ & $-6.291^{+0.007}_{-0.007}$  \\ 
\texttt{ATMO2020 NEQ weak} & $899$ & $461.1^{+2.4}_{-2.5}$ & $4.799^{+0.038}_{-0.039}$ & (0) & ($0.55$) & $\dots$ & ($3.40^{+0.08}_{-0.08}$) & $1.027^{+0.017}_{-0.016}$ & $-18.41^{+0.05}_{-0.05}$ & $-6.326^{+0.005}_{-0.005}$  \\ 
\hline   
\multicolumn{10}{c}{equilibrium chemistry + clouds}   \\ 
\hline   
\texttt{Linder19 Cloudy} & $390$ & $676.1^{+2.8}_{-3.2}$ & $3.251^{+0.027}_{-0.036}$ & $-0.396^{+0.006}_{-0.003}$ & ($0.55$) & $0.78^{+0.03}_{-0.03}$ & $\dots$ & $0.575^{+0.005}_{-0.005}$ & $-18.08^{+0.02}_{-0.02}$ & $-6.186^{+0.006}_{-0.006}$  \\ 
\texttt{Morley12} & $1015$ & $570.0^{+4.8}_{-4.9}$ & $4.718^{+0.053}_{-0.055}$ & (0) & ($0.497$) & $4.97^{+0.02}_{-0.03}$ & $\dots$ & $0.622^{+0.010}_{-0.010}$ & $-18.02^{+0.02}_{-0.02}$ & $-6.405^{+0.005}_{-0.005}$  \\ 
\texttt{Morley14}\tablenotemark{\scriptsize e} & $1538$ & $449.9^{+0.1}_{-0.1}$ & $4.204^{+0.034}_{-0.035}$ & (0) & ($0.497$) & (5) & $\dots$ & $1.024^{+0.004}_{-0.004}$ & $-17.99^{+0.02}_{-0.02}$ & $-6.360^{+0.004}_{-0.004}$  \\ 
\hline   
\multicolumn{10}{c}{equilibrium chemistry + no clouds}   \\ 
\hline   
\texttt{LB23 Clear CEQ} (M1)\tablenotemark{\scriptsize f} & $906$ & $561.7^{+0.7}_{-0.8}$ & $4.630^{+0.013}_{-0.016}$ & $-0.262^{+0.012}_{-0.012}$ & (0.537) & $\dots$ & $\dots$ & $0.631^{+0.004}_{-0.004}$ & $-18.10^{+0.02}_{-0.02}$ & $-6.408^{+0.004}_{-0.004}$  \\ 
\texttt{LB23 Clear CEQ} (M2)\tablenotemark{\scriptsize f} & $910$ & $559.6^{+0.7}_{-0.7}$ & $4.415^{+0.019}_{-0.012}$ & $-0.312^{+0.012}_{-0.013}$ & (0.537) & $\dots$ & $\dots$ & $0.633^{+0.004}_{-0.004}$ & $-18.12^{+0.03}_{-0.02}$ & $-6.411^{+0.004}_{-0.004}$  \\ 
\texttt{Linder19 Clear} & $935$ & $487.5^{+1.6}_{-1.6}$ & $3.218^{+0.052}_{-0.050}$ & $-0.394^{+0.010}_{-0.005}$ & ($0.55$) & $\dots$ & $\dots$ & $0.864^{+0.008}_{-0.009}$ & $-18.37^{+0.04}_{-0.05}$ & $-6.378^{+0.004}_{-0.004}$  \\ 
\texttt{ATMO2020 CEQ} & $993$ & $493.0^{+2.0}_{-1.9}$ & $5.179^{+0.042}_{-0.041}$ & (0) & ($0.55$) & $\dots$ & $\dots$ & $0.835^{+0.008}_{-0.008}$ & $-18.18^{+0.03}_{-0.03}$ & $-6.387^{+0.004}_{-0.004}$  \\ 
\texttt{Sonora Bobcat} & $1298$ & $530.3^{+2.6}_{-2.7}$ & $5.493^{+0.005}_{-0.010}$ & $0.102^{+0.020}_{-0.021}$ & ($0.458$) & $\dots$ & $\dots$ & $0.701^{+0.008}_{-0.008}$ & $-18.19^{+0.03}_{-0.03}$ & $-6.414^{+0.004}_{-0.004}$  \\ 
\enddata 
\tablenotetext{a}{The Sonora Elf Owl models are not used because the synthetic spectra (with a wavelength cutoff at 15~$\mu$m) do not cover the full wavelength of the $W3$ filter response.}  
\tablenotetext{b}{This column lists the BIC value of each model grid relative to that of the \texttt{PH$_{3}$-free ATMO2020++} models.}  
\tablenotetext{c}{Values inside parentheses are fixed by the model grids. In particular, the $\log{(K_{\rm zz})}$ values of the \texttt{ATMO2020}, \texttt{ATMO2020++}, and \texttt{PH$_{3}$-free ATMO2020++} modeling results are linearly interpolated from the inferred $\log{(g)}$ based on Figure~1 of Phillips et al. (2021). }  
\tablenotetext{d}{The bolometric luminosity is computed based on Equation~\ref{eq:lbol} that accounts for the offsets between observed fluxes and the fitted models}  
\tablenotetext{e}{The inferred $T_{\rm eff}$ based on \texttt{Morley14} models is pinned at the maximum grid value at 450~K.}  
\tablenotetext{f}{The parameter posteriors inferred by the \texttt{LB23 Clear CEQ} grid exhibit two modes, with the corresponding results labeled as ``M1'' and ``M2''.   }  
\end{deluxetable*} 
} 


==> COCONUTS2b_evo_params.tex <==
{ 
\begin{deluxetable*}{lccccccccccc}
\setlength{\tabcolsep}{2pt} 
\tablecaption{Evolution-based properties of COCONUTS-2b based on $L_{\rm bol}$ and age} \label{tab:evoparams} 
\tablehead{ \multicolumn{1}{l}{Evolution Models} &  \multicolumn{2}{c}{$T_{\rm eff}$} &  \multicolumn{1}{c}{} &  \multicolumn{2}{c}{$R$} &  \multicolumn{1}{c}{} &  \multicolumn{2}{c}{$\log{g}$} &  \multicolumn{1}{c}{} &  \multicolumn{2}{c}{$M$} \\ 
\cline{2-3} \cline{5-6} \cline{8-9} \cline{11-12} 
\multicolumn{1}{l}{}  &  \multicolumn{1}{c}{Median$\pm 1\sigma$} &  \multicolumn{1}{c}{$3\sigma$ C. I.} &  \multicolumn{1}{c}{}  &  \multicolumn{1}{c}{Median$\pm 1\sigma$} &  \multicolumn{1}{c}{$3\sigma$ C. I.} &  \multicolumn{1}{c}{}  &  \multicolumn{1}{c}{Median$\pm 1\sigma$} &  \multicolumn{1}{c}{$3\sigma$ C. I.} &  \multicolumn{1}{c}{}  &  \multicolumn{1}{c}{Median$\pm 1\sigma$} &  \multicolumn{1}{c}{$3\sigma$ C. I.} \\ 
\multicolumn{1}{l}{}  &  \multicolumn{1}{c}{(K)} &  \multicolumn{1}{c}{(K)} &  \multicolumn{1}{c}{}  &  \multicolumn{1}{c}{(R$_{\rm Jup}$)} &  \multicolumn{1}{c}{(R$_{\rm Jup}$)} &  \multicolumn{1}{c}{}  &  \multicolumn{1}{c}{(dex)} &  \multicolumn{1}{c}{(dex)} &  \multicolumn{1}{c}{}  &  \multicolumn{1}{c}{(M$_{\rm Jup}$)} &  \multicolumn{1}{c}{(M$_{\rm Jup}$)}  } 
\startdata 
hot-start ATMO2020  &  $490^{+47}_{-52}$  &  ($416$, $577$)  &  &  $1.09^{+0.03}_{-0.04}$  &  ($1.05$, $1.16$)  &    &  $4.21^{+0.18}_{-0.14}$  &   ($3.8$, $4.5$)   &  &  $8^{+2}_{-2}$  &   ($3$, $12$)  \\ 
hot-start Sonora Bobcat [M/H]$=+0.5$  &  $488^{+47}_{-52}$  &  ($413$, $575$)  &  &  $1.10^{+0.03}_{-0.04}$  &  ($1.05$, $1.17$)  &    &  $4.20^{+0.19}_{-0.14}$  &   ($3.8$, $4.4$)   &  &  $8^{+2}_{-2}$  &   ($3$, $12$)  \\ 
hot-start Sonora Bobcat [M/H]$=0$  &  $485^{+47}_{-52}$  &  ($411$, $570$)  &  &  $1.12^{+0.03}_{-0.04}$  &  ($1.07$, $1.19$)  &    &  $4.18^{+0.18}_{-0.14}$  &   ($3.8$, $4.4$)   &  &  $8^{+2}_{-2}$  &   ($3$, $12$)  \\ 
hot-start Sonora Bobcat [M/H]$=-0.5$  &  $484^{+46}_{-51}$  &  ($410$, $569$)  &  &  $1.12^{+0.03}_{-0.04}$  &  ($1.07$, $1.19$)  &    &  $4.16^{+0.19}_{-0.13}$  &   ($3.7$, $4.4$)   &  &  $7^{+2}_{-2}$  &   ($3$, $11$)  \\ 
cold-start Sonora Bobcat [M/H]$=0$  &  $466^{+33}_{-47}$  &  ($411$, $561$)  &  &  $1.12^{+0.03}_{-0.04}$  &  ($1.07$, $1.18$)  &    &  $4.17^{+0.17}_{-0.10}$  &   ($3.8$, $4.3$)   &  &  $7^{+2}_{-2}$  &   ($3$, $10$)  \\ 
\hline 
{\bf Adopted}\tablenotemark{\scriptsize a}  &  $483^{+44}_{-53}$  &  ($411$, $575$)  &  &  $1.11^{+0.03}_{-0.04}$  &  ($1.05$, $1.19$)  &    &  $4.19^{+0.18}_{-0.13}$  &   ($3.7$, $4.4$)   &  &  $8^{+2}_{-2}$  &   ($3$, $12$)  \\ 
\enddata 
\tablenotetext{a}{The adopted parameters are inferred from the concatenated chains of all the evolution models (Section~\ref{subsubsec:tgrm}).}  
\end{deluxetable*} 
} 

